Optimal Interactive Learning on the Job via Facility Location Planning

Collaborative robots must continually adapt to novel tasks and user preferences without overburdening the user. While prior interactive robot learning methods aim to reduce human effort, they are typically limited to single-task scenarios and are not well-suited for sustained, multi-task collaboration. We propose COIL (Cost-Optimal Interactive Learning) -- a multi-task interaction planner that minimizes human effort across a sequence of tasks by strategically selecting among three query types (skill, preference, and help). When user preferences are known, we formulate COIL as an uncapacitated facility location (UFL) problem, which enables bounded-suboptimal planning in polynomial time using off-the-shelf approximation algorithms. We extend our formulation to handle uncertainty in user preferences by incorporating one-step belief space planning, which uses these approximation algorithms as subroutines to maintain polynomial-time performance. Simulated and physical experiments on manipulation tasks show that our framework significantly reduces the amount of work allocated to the human while maintaining successful task completion.

==> includes/n_archive.tex <==
\subsection{Interaction MDP}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{imgs/tasksetup.png}
    \caption{Task setup}
    \label{fig:tasksetup}
\end{figure}

In this toy environment, the robot is asked to help a human place a set of objects to their correct goal locations while optimizing reward functions that reflect the human's preferences. There exist four types of objects \{glass-mug, metal-mug, spoon, fork\}. These objects must be placed in one of two goal locations $G_1$ and $G_2$, which have fixed locations in the top right and bottom right corner positions, respectively. The human preference for the goal location for each object is captured by a reward function $R_{goal}$ and their preference for the grasp used by the robot is captured by a reward function $R_{grasp}$.
Both these reward functions are unknown to the robot. However, the robot may query human feedback through multiple interaction types in order to learn  the rewards.
% both the reward itself and skills needed to execute actions which maximize the reward.

We model this interaction as a single-agent MDP, called the \textit{Interaction MDP}, defined by the tuple $M = \langle \SS, \AA, \TT, R, P_0\rangle$. $S$ represents the set of states and $P_0$ the initial state distribution. The initial state of the environment begins with $n_A$ and $n_B$ types of each object placed in random locations. For this toy environment, each state $s\in S$ is a vector [$(type_i, x_i, y_i) \forall$ object $i$ not in any goal, number of typeA objects in $G_1$, number of typeB objects in $G_1$, number of typeA objects in $G_2$, number of typeB objects in $G_2$].

The robot $rob$ does not begin with access to $R$. $R = w^{*T} \phi(s)$ is parameterized by a weight vector $w^*$, known only to the human $hum$, which linearly combines a set of state features, where $\phi$ is a state featurization function. $\phi(s)=$ [number of typeA objects in $G_1$, number of typeB objects in $G_1$, number of typeA objects in $G_2$, number of typeB objects in $G_2$]. And $w^* = [1, -1, -1, 1]$, which means the correct placement of items is all typeA should be in $G_1$, and all typeB objects should be in $G_2$.

The action space $\AA = \{a_{rob}, a_{demo}, a_{pref}\}$. There are 3 actions:
\begin{itemize}
    \item $a_{rob}$: robot attempts a task with cost $c_{rob}$.
    \item $a_{hum}$: human attempts a task with cost $c_{hum}$. \MZ{I'm going to leave this out because this seems to give the same info as a demo.} \PC{Does this action imply the robot doesn't learn from the human's attempt? (As opposed to a demo.)}
    \item $a_{demo}$: human gives a physical demo to the robot with cost $c_{demo}$.
    \item $a_{pref}$: human answers a preference query with cost $c_{pref}$.
\end{itemize}
Although the set contains actions performed by the human and robot, we do not model this as a two-agent MDP because all actions are elicited by the robot. In performing $a_{demo}, a_{pref}$, the robot would ask the human to act in the task for a timestep (the human moves one object to a goal), request a demonstration, or request an answer to a preference query. We will discuss the specifics of these action types in detail in the next sections. 

$\TT(s'|s,a)$ represents the transition probability to state $s'$ when taking action $a$ in state $s$. In the interaction MDP, we will model every action deterministically in $\TT$ with the following assumptions:
\begin{itemize}
    \item Action $a$ will be successful with probability 1. 
    \item The human will provide an answer to either query $a_{demo}$ or $a_{pref}$ with probability 1.
    \item The robot's inability to perform actions will not be modeled in $\TT$, but modeled through preconditions used in the determining the robot's optimization objective.
\end{itemize}

\subsection{Detailing Actions in the Interaction MDP leads us to skill MDPs}
When the agent performs $a_{rob}$, the robot attempts the task by performing one of two skills \{move nearest typeA object to the appropriate goal, move nearest typeB object to the appropriate goal\}. 

When the agent performs $a_{demo}$, the robot asks for the human to demonstrate execution of one of two skills \{move nearest typeA object to the appropriate goal, move nearest typeB object to the appropriate goal\}. 

When the agent performs $a_{pref}$, the robot asks one of two queries \{should the nearest typeA object go in $G_1$ or $G_2$?, should the nearest typeB object go in $G_1$ or $G_2$?\}.

\subsection{Skill MDP}
The types of capabilities required are \{move nearest typeA object, move nearest typeB object\}. We model these capabilities as a library of skills $\Pi_w = \{\pi_{1,w},\ldots,\pi_{n,w}\}$. Each skill consists of a control policy $\pi$ and its precondition \textsc{Pre}(s) which models the probability of success of the policy when applied at a state $s$.

In our case, $\pi_{A,w}$= move the nearest typeA object to the appropriate goal under $w$ and $\pi_{B,w}$= move the nearest typeB object to the appropriate goal under $w$.

$\pi_{i,w}$ is the solution to a \textit{skill MDP}, defined by the tuple $M_{i,w} = \langle \SS, \AA_i, \TT_i, R_i, P_0\rangle$. $\SS$ is identical to the states of the interaction MDP. However, $\AA_i$ is the set \{up, down, left, right, pickup typeA object, place typeA object\}, and the transitions $\TT_i$ deterministically reflect these movements. $R_i$ is parameterized by $w$ and rewards the agent for placing an object in a particular goal. The skill MDP ends when an object is placed in a goal, and thus only the object with the minimum step cost will be moved.

In practice, $\pi_{i,w}$ is a behaviorally cloned policy learned from human demonstrations which we assume come from the human solving $M_{i,w}$. We pass as input to the policy the current state, object type and location to be picked up: $\pi_{i,w}(s, (o,x,y))$, and rollout the policy to completion.

\subsubsection{Skill Preconditions}
The preconditions for each skill are represented as a Gaussian Process.
\MZ{Fill out GP specifications (input requested from Shivam)}


\subsection{Learning from Demonstrations and Preferences}
We begin with two candidate $w$ vectors. $[w_1, w_2]$ where $w_1 = [1, -1, -1, 1]$ (this is $w^*$), and $w_2 = [-1, 1, 1, -1]$. We begin with a uniform prior over the two weight vectors $b=[P(w_1), P(w_2)] =[0.5, 0.5]$.

\paragraph{Preferences}
A query from the robot looks like $\{(o_A, x_A, y_A), \{G_1, G_2\}\}\rightarrow$ should object of type A in position $(x_A, y_A)$ go into $G_1$ or $G_2$? or $\{(o_B, x_B, y_B), \{G_1, G_2\}\} \rightarrow$ should object of type B in position $(x_B, y_B)$ go into $G_1$ or $G_2$? 

The likelihood is defined
$$P(G_p > G_q| w_i, (o_j, x_j, y_j)) = \frac{e^{\beta w_i^T \phi(s'\rightarrow o_j in G_p)}}{e^{\beta w_i^T \phi(s'\rightarrow o_j in G_p)} + e^{\beta w_i^T \phi(s'\rightarrow o_j in G_q)}}$$

The posterior becomes
\begin{align}
b(w_i)= & P(w_i| G_p > G_q, (o_j, x_j, y_j) \\
&\propto P(G_p > G_q| w_i, (o_j, x_j, y_j)) P(w_i)
\end{align}

\paragraph{Demonstrations}
A query from the robot looks like $\{(o_A, x_A, y_A), \{G_1, G_2\}\}\rightarrow$ request human to move object of type A in position $(x_A, y_A)$ into $G_1$ or $G_2$ or $\{(o_B, x_B, y_B), \{G_1, G_2\}\} \rightarrow$ request human to move object of type B in position $(x_B, y_B)$ into $G_1$ or $G_2$.

The robot picks $(o_j, x_j, y_j), \{G_p, G_q\}$ and receives demonstration $\xi = \{(o_j, x_j, y_j), ..., (o_j, x_{G_p}, y_{G_p}) \}$, moving object $(o_j, x_j, y_j)$ to goal $G_p$.

First, the policy $\pi_{i,w}$ is updated $\pi_{i,w} \leftarrow BC(\pi_{i,w}, \xi)$. Then, the posterior beliefs $b$ are updates in the same way as the preferences $$P(w_i| G_p > G_q, (o_j, x_j, y_j) \propto P(G_p > G_q| w_i, (o_j, x_j, y_j)) P(w_i)$$.


\subsection{Acting in the Environment}

The robot takes actions in $s$ which maximize the expected reward $J(a, s)$:
$$a_{rob} \leftarrow arg\max_{a\in \AA} J(a, s)$$

% We'll say that $\tau_A \sim \pi_{A}$ is the trajectory performed when $\pi_A(s)$ 
$J(a_{rob}, s) = arg\max_{\pi_A, \pi_B} -C(a_{rob}) + \{\EE[R]_{\sim b} (\pi_{A}(s) \cdot Pre(A,s)), \EE[R]_{\sim b} (\pi_{B}(s) \cdot Pre(B,s))  \}$

$J(a_{demo}, s) = arg\max_{\pi_A, \pi_B} -C(a_{demo}) + \{\EE[R]_{\sim b'} (\pi'_{A}(s) \cdot Pre(A,s)), \EE[R]_{\sim b} (\pi'_{B}(s) \cdot Pre(B,s))  \}$ where $b'$ and $\pi'$ are the updated beliefs and policy.

$J(a_{pref}, s) = arg\max_{\pi_A, \pi_B} -C(a_{pref}) +\gamma \{\EE[R]_{\sim b'} (\pi_{A}(s) \cdot Pre(A,s)), \EE[R]_{\sim b} (\pi_{B}(s) \cdot Pre(B,s))  \}$ where $b'$ is the updated belief.

